DI-BENCH: Benchmarking Large Language Models on Dependency Inference with Testable Repositories at Scale

Large Language Models have advanced automated software development, however, it remains a challenge to correctly infer dependencies, namely, identifying the internal components and external packages required for a repository to successfully run. Existing studies highlight that dependency-related issues cause over 40\% of observed runtime errors on the generated repository. To address this, we introduce DI-BENCH, a large-scale benchmark and evaluation framework specifically designed to assess LLMs' capability on dependency inference. The benchmark features 581 repositories with testing environments across Python, C#, Rust, and JavaScript. Extensive experiments with textual and execution-based metrics reveal that the current best-performing model achieves only a 42.9% execution pass rate, indicating significant room for improvement. DI-BENCH establishes a new viewpoint for evaluating LLM performance on repositories, paving the way for more robust end-to-end software synthesis.

==> intro.tex <==
\section{Introduction}

Large Language Models (LLMs) have revolutionized automated software development, scaling from local code completion~\cite{copilot} to entire repository-level code synthesis~\cite{openhands, chatdev, ibrahimzada2024repository}. Recent advancements have enabled these models not only to generate source code but also to orchestrate high-level tasks such as repository configuration, toolchain selection, and code translation. A pivotal yet often overlooked step in this process is ensuring that generated repositories are fully executable. This requires accurate inference and integration of all necessary dependencies, both internal (across project components) and external (from package ecosystems). Without robust dependency inference, even the most sophisticated repository-level code generation solutions risk failing at runtime, impeding further iteration, comprehensive evaluation, and reliable deployment.

As illustrated in Figure~\ref{fig:dep}, dependency inference involves understanding the intricate relationships within the codebase and mapping out the external packages required for execution. Such dependencies are typically documented in configuration files (see Appendix~\ref{appdix:config}). Correctly reconstructing these relationships is a foundational capability: it not only ensures that code generation tools produce functional and self-contained repositories, but it also informs deeper reasoning about project architecture and build systems~\cite{pypi, crates}. Consequently, mastering dependency inference is a critical leap forward for enabling robust, end-to-end software synthesis and maintenance.

Despite the significance of dependency inference, current LLM-based approaches struggle in this area. Works like ChatDev~\cite{chatdev} and DevBench~\cite{devbench}—pioneers in repository-level generation using multi-agent LLM systems—have reported that dependency-related issues (e.g., missing or incorrectly specified modules) account for over 40\% of their observed runtime errors. These challenges highlight the difficulty that state-of-the-art models face in accurately navigating build systems and package repositories. Although existing repository-level benchmarks such as SWEBench~\cite{swebench}, RepoBench~\cite{repobench}, and DevBench~\cite{devbench} offer valuable insights into a model’s ability to handle large contexts and generate code at scale, none focuses on systematically evaluating dependency inference capabilities.

To address this critical gap, we introduce \bench{}, the first comprehensive repository-level benchmark dedicated specifically to dependency inference. \bench{} comprises 600 repositories—including 400 regular-sized and 200 large—across four popular programming languages (Python, C#, Rust, and JavaScript). Each repository is carefully curated to assess a model’s ability to identify both internal and external dependencies. We pair this dataset with a rigorous, multi-faceted evaluation framework. Beyond measuring textual matching accuracy between model-generated and ground-truth dependencies, we also propose a novel CI-based execution evaluation: we reuse each repository’s original Continuous Integration (CI) scripts as automated test harnesses. This approach enables scalable and objective assessment of end-to-end executability, eliminating the costly and error-prone need for manual environment setup.

In summary, our contributions are as follows:
\begin{itemize}[leftmargin=*] 
    \item \textbf{\bench{} Benchmark:} We introduce a pioneering, dependency-focused benchmark featuring 600 repositories (400 regular and 200 large) spanning 4 popular programming languages. This resource establishes a new standard for evaluating LLMs' dependency inference capabilities in realistic, repository-scale scenarios. 
    \item \textbf{Dual-Use CI Infrastructure:} We leverage CI workflows not only to identify well-maintained, executable repositories during dataset curation but also to serve as a reliable, fully automated test environment. By using developer-provided CI scripts, we ensure that dependency checks remain robust, scalable, and faithful to real-world development practices. 
    \item \textbf{Granular Evaluation Metrics:} We combine coarse-grained runtime executability measures with fine-grained precision and recall on inferred dependency items. This dual-layered approach yields richer insights into model performance, enabling systematic analysis of both functional correctness and textual accuracy. 
\end{itemize}
By foregrounding dependency inference as a first-class challenge in repository-level code generation and introducing a dedicated benchmark to measure it, our work lays the groundwork for advancing LLM capabilities toward end-to-end, reliable software synthesis.
